Traffic Signal Optimization on a Square Lattice with Quantum Annealing

The spread of intelligent transportation systems in urban cities has caused heavy computational loads, requiring a novel architecture for managing large-scale traffic. In this study, we develop a method for globally controlling traffic signals arranged on a square lattice by means of a quantum annealing machine, namely the D-Wave quantum annealer. We first formulate a signal optimization problem that minimizes the imbalance of traffic flows in two orthogonal directions. Then we reformulate this problem as an Ising Hamiltonian, which is fully compatible with quantum annealers. The new control method is compared with a conventional local control method for a large 50-by-50 city, and the results exhibit the superiority of our global control method in suppressing traffic imbalance over wide parameter ranges. Furthermore, the solutions to the global control method obtained with the quantum annealing machine are better than those obtained with conventional simulated annealing. In addition, we prove analytically that the local and the global control methods converge at the limit where cars have equal probabilities for turning and going straight. These results are verified with numerical experiments.

==> macro.tex <==
\usepackage{color}

\newcommand\rev[1]{\textcolor{red}{{#1}}}

\newcommand{\dif}{\mathrm{d}}
\newcommand{\E}{\mathrm{E}}


%%  微分
\newcommand{\drv}[2]{\frac{\dif #1}{\dif #2}}

%%  偏微分
\newcommand{\pdrv}[2]{\frac{\partial #1}{\partial #2}}

%%  変分
\newcommand{\ddrv}[2]{\frac{\delta #1}{\delta #2}}

%% 内積
\newcommand{\ip}[1]{\left\langle #1 \right\rangle}

%% argmin, argmax
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

%% caligraphic fonts
\newcommand{\calA}{{\mathcal A}}
\newcommand{\calB}{{\mathcal B}}
\newcommand{\calC}{{\mathcal C}}
\newcommand{\calD}{{\mathcal D}}
\newcommand{\calE}{{\mathcal E}}
\newcommand{\calF}{{\mathcal F}}
\newcommand{\calG}{{\mathcal G}}
\newcommand{\calH}{{\mathcal H}}
\newcommand{\calI}{{\mathcal I}}
\newcommand{\calJ}{{\mathcal J}}
\newcommand{\calK}{{\mathcal K}}
\newcommand{\calL}{{\mathcal L}}
\newcommand{\calM}{{\mathcal M}}
\newcommand{\calN}{{\mathcal N}}
\newcommand{\calO}{{\mathcal O}}
\newcommand{\calP}{{\mathcal P}}
\newcommand{\calQ}{{\mathcal Q}}
\newcommand{\calR}{{\mathcal R}}
\newcommand{\calS}{{\mathcal S}}
\newcommand{\calT}{{\mathcal T}}
\newcommand{\calU}{{\mathcal U}}
\newcommand{\calV}{{\mathcal V}}
\newcommand{\calW}{{\mathcal W}}
\newcommand{\calX}{{\mathcal X}}
\newcommand{\calY}{{\mathcal Y}}
\newcommand{\calZ}{{\mathcal Z}}

%% script fonts
\newcommand{\scrA}{{\mathscr A}}
\newcommand{\scrB}{{\mathscr B}}
\newcommand{\scrC}{{\mathscr C}}
\newcommand{\scrD}{{\mathscr D}}
\newcommand{\scrE}{{\mathscr F}}
\newcommand{\scrF}{{\mathscr F}}
\newcommand{\scrG}{{\mathscr G}}
\newcommand{\scrH}{{\mathscr H}}
\newcommand{\scrI}{{\mathscr I}}
\newcommand{\scrJ}{{\mathscr J}}
\newcommand{\scrK}{{\mathscr K}}
\newcommand{\scrL}{{\mathscr L}}
\newcommand{\scrM}{{\mathscr M}}
\newcommand{\scrN}{{\mathscr N}}
\newcommand{\scrO}{{\mathscr O}}
\newcommand{\scrP}{{\mathscr P}}
\newcommand{\scrQ}{{\mathscr Q}}
\newcommand{\scrR}{{\mathscr R}}
\newcommand{\scrS}{{\mathscr S}}
\newcommand{\scrT}{{\mathscr T}}
\newcommand{\scrU}{{\mathscr U}}
\newcommand{\scrV}{{\mathscr V}}
\newcommand{\scrW}{{\mathscr W}}
\newcommand{\scrX}{{\mathscr X}}
\newcommand{\scrY}{{\mathscr Y}}
\newcommand{\scrZ}{{\mathscr Z}}

%% blackborad fonts
\newcommand{\bbA}{{\mathbb A}}
\newcommand{\bbB}{{\mathbb B}}
\newcommand{\bbC}{{\mathbb C}}
\newcommand{\bbD}{{\mathbb D}}
\newcommand{\bbE}{{\mathbb E}}
\newcommand{\bbF}{{\mathbb F}}
\newcommand{\bbG}{{\mathbb G}}
\newcommand{\bbH}{{\mathbb H}}
\newcommand{\bbI}{{\mathbb I}}
\newcommand{\bbJ}{{\mathbb J}}
\newcommand{\bbK}{{\mathbb K}}
\newcommand{\bbL}{{\mathbb L}}
\newcommand{\bbM}{{\mathbb M}}
\newcommand{\bbN}{{\mathbb N}}
\newcommand{\bbO}{{\mathbb O}}
\newcommand{\bbP}{{\mathbb P}}
\newcommand{\bbQ}{{\mathbb Q}}
\newcommand{\bbR}{{\mathbb R}}
\newcommand{\bbS}{{\mathbb S}}
\newcommand{\bbT}{{\mathbb T}}
\newcommand{\bbU}{{\mathbb U}}
\newcommand{\bbV}{{\mathbb V}}
\newcommand{\bbW}{{\mathbb W}}
\newcommand{\bbX}{{\mathbb X}}
\newcommand{\bbY}{{\mathbb Y}}
\newcommand{\bbZ}{{\mathbb Z}}

%% bold italic

\newcommand{\bma}{\mbox{\boldmath $a$}}
\newcommand{\bmb}{\mbox{\boldmath $b$}}
\newcommand{\bmc}{\mbox{\boldmath $c$}}
\newcommand{\bmd}{\mbox{\boldmath $d$}}
\newcommand{\bme}{\mbox{\boldmath $e$}}
\newcommand{\bmf}{\mbox{\boldmath $f$}}
\newcommand{\bmg}{\mbox{\boldmath $g$}}
\newcommand{\bmh}{\mbox{\boldmath $h$}}
\newcommand{\bmi}{\mbox{\boldmath $i$}}
\newcommand{\bmj}{\mbox{\boldmath $j$}}
\newcommand{\bmk}{\mbox{\boldmath $k$}}
\newcommand{\bml}{\mbox{\boldmath $l$}}
\newcommand{\bmm}{\mbox{\boldmath $m$}}
\newcommand{\bmn}{\mbox{\boldmath $n$}}
\newcommand{\bmo}{\mbox{\boldmath $o$}}
\newcommand{\bmp}{\mbox{\boldmath $p$}}
\newcommand{\bmq}{\mbox{\boldmath $q$}}
\newcommand{\bmr}{\mbox{\boldmath $r$}}
\newcommand{\bms}{\mbox{\boldmath $s$}}
\newcommand{\bmt}{\mbox{\boldmath $t$}}
\newcommand{\bmu}{\mbox{\boldmath $u$}}
\newcommand{\bmv}{\mbox{\boldmath $v$}}
\newcommand{\bmw}{\mbox{\boldmath $w$}}
\newcommand{\bmx}{\mbox{\boldmath $x$}}
\newcommand{\bmy}{\mbox{\boldmath $y$}}
\newcommand{\bmz}{\mbox{\boldmath $z$}}
\newcommand{\bmsigma}{\mbox{\boldmath $\sigma$}}
\newcommand{\bmlambda}{\mbox{\boldmath $\lambda$}}

\newcommand{\bmA}{\mbox{\boldmath $A$}}
\newcommand{\bmB}{\mbox{\boldmath $B$}}
\newcommand{\bmC}{\mbox{\boldmath $C$}}
\newcommand{\bmD}{\mbox{\boldmath $D$}}
\newcommand{\bmE}{\mbox{\boldmath $E$}}
\newcommand{\bmF}{\mbox{\boldmath $F$}}
\newcommand{\bmG}{\mbox{\boldmath $G$}}
\newcommand{\bmH}{\mbox{\boldmath $H$}}
\newcommand{\bmI}{\mbox{\boldmath $I$}}
\newcommand{\bmJ}{\mbox{\boldmath $J$}}
\newcommand{\bmK}{\mbox{\boldmath $K$}}
\newcommand{\bmL}{\mbox{\boldmath $L$}}
\newcommand{\bmM}{\mbox{\boldmath $M$}}
\newcommand{\bmN}{\mbox{\boldmath $N$}}
\newcommand{\bmO}{\mbox{\boldmath $O$}}
\newcommand{\bmP}{\mbox{\boldmath $P$}}
\newcommand{\bmQ}{\mbox{\boldmath $Q$}}
\newcommand{\bmR}{\mbox{\boldmath $R$}}
\newcommand{\bmS}{\mbox{\boldmath $S$}}
\newcommand{\bmT}{\mbox{\boldmath $T$}}
\newcommand{\bmU}{\mbox{\boldmath $U$}}
\newcommand{\bmV}{\mbox{\boldmath $V$}}
\newcommand{\bmW}{\mbox{\boldmath $W$}}
\newcommand{\bmX}{\mbox{\boldmath $X$}}
\newcommand{\bmY}{\mbox{\boldmath $Y$}}
\newcommand{\bmZ}{\mbox{\boldmath $Z$}}

\newcommand{\frakA}{{\mathfrak A}}
\newcommand{\frakB}{{\mathfrak B}}
\newcommand{\frakC}{{\mathfrak C}}
\newcommand{\frakD}{{\mathfrak D}}
\newcommand{\frakE}{{\mathfrak E}}
\newcommand{\frakF}{{\mathfrak F}}
\newcommand{\frakG}{{\mathfrak G}}
\newcommand{\frakH}{{\mathfrak H}}
\newcommand{\frakI}{{\mathfrak I}}
\newcommand{\frakJ}{{\mathfrak J}}
\newcommand{\frakK}{{\mathfrak K}}
\newcommand{\frakL}{{\mathfrak L}}
\newcommand{\frakM}{{\mathfrak M}}
\newcommand{\frakN}{{\mathfrak N}}
\newcommand{\frakO}{{\mathfrak O}}
\newcommand{\frakP}{{\mathfrak P}}
\newcommand{\frakQ}{{\mathfrak Q}}
\newcommand{\frakR}{{\mathfrak R}}
\newcommand{\frakS}{{\mathfrak S}}
\newcommand{\frakT}{{\mathfrak T}}
\newcommand{\frakU}{{\mathfrak U}}
\newcommand{\frakV}{{\mathfrak V}}
\newcommand{\frakW}{{\mathfrak W}}
\newcommand{\frakX}{{\mathfrak X}}
\newcommand{\frakY}{{\mathfrak Y}}
\newcommand{\frakZ}{{\mathfrak Z}}

\newcommand{\rma}{{\mathrm a}}
\newcommand{\rmb}{{\mathrm b}}
\newcommand{\rmc}{{\mathrm c}}
\newcommand{\rmd}{{\mathrm d}}
\newcommand{\rme}{{\mathrm e}}
\newcommand{\rmf}{{\mathrm f}}
\newcommand{\rmg}{{\mathrm g}}
\newcommand{\rmh}{{\mathrm h}}
\newcommand{\rmi}{{\mathrm i}}
\newcommand{\rmj}{{\mathrm j}}
\newcommand{\rmk}{{\mathrm k}}
\newcommand{\rml}{{\mathrm l}}
\newcommand{\rmm}{{\mathrm m}}
\newcommand{\rmn}{{\mathrm n}}
\newcommand{\rmo}{{\mathrm o}}
% \newcommand{\rmp}{{\mathrm p}}
\newcommand{\rmq}{{\mathrm q}}
\newcommand{\rmr}{{\mathrm r}}
\newcommand{\rms}{{\mathrm s}}
\newcommand{\rmt}{{\mathrm t}}
\newcommand{\rmu}{{\mathrm u}}
\newcommand{\rmv}{{\mathrm v}}
\newcommand{\rmw}{{\mathrm w}}
\newcommand{\rmx}{{\mathrm x}}
\newcommand{\rmy}{{\mathrm y}}
\newcommand{\rmz}{{\mathrm z}}

\newcommand{\rmA}{{\mathrm A}}
\newcommand{\rmB}{{\mathrm B}}
\newcommand{\rmC}{{\mathrm C}}
\newcommand{\rmD}{{\mathrm D}}
\newcommand{\rmE}{{\mathrm E}}
\newcommand{\rmF}{{\mathrm F}}
\newcommand{\rmG}{{\mathrm G}}
\newcommand{\rmH}{{\mathrm H}}
\newcommand{\rmI}{{\mathrm I}}
\newcommand{\rmJ}{{\mathrm J}}
\newcommand{\rmK}{{\mathrm K}}
\newcommand{\rmL}{{\mathrm L}}
\newcommand{\rmM}{{\mathrm M}}
\newcommand{\rmN}{{\mathrm N}}
\newcommand{\rmO}{{\mathrm O}}
\newcommand{\rmP}{{\mathrm P}}
\newcommand{\rmQ}{{\mathrm Q}}
\newcommand{\rmR}{{\mathrm R}}
\newcommand{\rmS}{{\mathrm S}}
\newcommand{\rmT}{{\mathrm T}}
\newcommand{\rmU}{{\mathrm U}}
\newcommand{\rmV}{{\mathrm V}}
\newcommand{\rmW}{{\mathrm W}}
\newcommand{\rmX}{{\mathrm X}}
\newcommand{\rmY}{{\mathrm Y}}
\newcommand{\rmZ}{{\mathrm Z}}


\newcommand{\tila}{{\tilde a}}
\newcommand{\tilb}{{\tilde b}}
\newcommand{\tilc}{{\tilde c}}
\newcommand{\tild}{{\tilde d}}
\newcommand{\tile}{{\tilde e}}
\newcommand{\tilf}{{\tilde f}}
\newcommand{\tilg}{{\tilde g}}
\newcommand{\tilh}{{\tilde h}}
\newcommand{\tili}{{\tilde i}}
\newcommand{\tilj}{{\tilde j}}
\newcommand{\tilk}{{\tilde k}}
\newcommand{\till}{{\tilde l}}
\newcommand{\tilm}{{\tilde m}}
\newcommand{\tiln}{{\tilde n}}
\newcommand{\tilo}{{\tilde o}}
\newcommand{\tilp}{{\tilde p}}
\newcommand{\tilq}{{\tilde q}}
\newcommand{\tilr}{{\tilde r}}
\newcommand{\tils}{{\tilde s}}
\newcommand{\tilt}{{\tilde t}}
\newcommand{\tilu}{{\tilde u}}
\newcommand{\tilv}{{\tilde v}}
\newcommand{\tilw}{{\tilde w}}
\newcommand{\tilx}{{\tilde x}}
\newcommand{\tily}{{\tilde y}}
\newcommand{\tilz}{{\tilde z}}
\newcommand{\tiltheta}{{\tilde \theta}}

\newcommand{\tilA}{{\tilde A}}
\newcommand{\tilB}{{\tilde B}}
\newcommand{\tilC}{{\tilde C}}
\newcommand{\tilD}{{\tilde D}}
\newcommand{\tilE}{{\tilde E}}
\newcommand{\tilF}{{\tilde F}}
\newcommand{\tilG}{{\tilde G}}
\newcommand{\tilH}{{\tilde H}}
\newcommand{\tilI}{{\tilde I}}
\newcommand{\tilJ}{{\tilde J}}
\newcommand{\tilK}{{\tilde K}}
\newcommand{\tilL}{{\tilde L}}
\newcommand{\tilM}{{\tilde M}}
\newcommand{\tilN}{{\tilde N}}
\newcommand{\tilO}{{\tilde O}}
\newcommand{\tilP}{{\tilde P}}
\newcommand{\tilQ}{{\tilde Q}}
\newcommand{\tilR}{{\tilde R}}
\newcommand{\tilS}{{\tilde S}}
\newcommand{\tilT}{{\tilde T}}
\newcommand{\tilU}{{\tilde U}}
\newcommand{\tilV}{{\tilde V}}
\newcommand{\tilW}{{\tilde W}}
\newcommand{\tilX}{{\tilde X}}
\newcommand{\tilY}{{\tilde Y}}
\newcommand{\tilZ}{{\tilde Z}}

